Speech language models lack important brain-relevant semantics

Despite known differences between reading and listening in the brain, recent work has shown that text-based language models predict both text-evoked and speech-evoked brain activity to an impressive degree. This poses the question of what types of information language models truly predict in the brain. We investigate this question via a direct approach, in which we systematically remove specific low-level stimulus features (textual, speech, and visual) from language model representations to assess their impact on alignment with fMRI brain recordings during reading and listening. Comparing these findings with speech-based language models reveals starkly different effects of low-level features on brain alignment. While text-based models show reduced alignment in early sensory regions post-removal, they retain significant predictive power in late language regions. In contrast, speech-based models maintain strong alignment in early auditory regions even after feature removal but lose all predictive power in late language regions. These results suggest that speech-based models provide insights into additional information processed by early auditory regions, but caution is needed when using them to model processing in late language regions. We make our code publicly available. [https://github.com/subbareddy248/speech-llm-brain]

==> ICLR_intro.tex <==
An explosion of recent work that investigates the alignment between the human brain and language models shows that text-based language models (e.g. GPT*, BERT, etc.) predict both text-evoked and speech-evoked brain activity to an impressive degree (text: \citep{toneva2019interpreting,schrimpf2021neural,goldstein2022shared,aw2022training,oota2022neural,lamarre2022attention,chen2023cortical}; speech: \citep{jain2018incorporating,caucheteux2020language,antonello2021low,vaidya2022self,millet2022toward,tuckute2022many,oota2022joint,oota2023neural,oota2023speech,chen2023cortical}. This observation holds across late language regions, which are thought to process both text- and speech-evoked language~\citep{deniz2019representation}, but also more surprisingly across early sensory cortices, which are shown to be modality-specific~\citep{deniz2019representation,chen2023cortical}. Since text-based language models are trained on written text~\citep{devlin2019bert,radford2019language,chung2022scaling}, their impressive performance at predicting the activity (also referred to as alignment) in early auditory cortices is puzzling. This raises the question of what types of information underlie the brain alignment of language models observed across brain regions.

\begin{figure*}[t] 
\centering
%\vspace{-1cm}
\begin{minipage}{0.45\textwidth}
\centering
\includegraphics[width=0.98\linewidth]    {images/Approach_part1.pdf}
\end{minipage}
\vline
\begin{minipage}{0.54\textwidth}
\centering
\includegraphics[width=0.98\linewidth]{images/Approach_part2.pdf}
\end{minipage}
\caption{A direct approach to test the effect of low-level stimulus features on the alignment between different types
of language models and brain recordings (reading vs. listening).}
\label{fig:approach}
\end{figure*}

In this work, we investigate this question via a direct approach (see Fig.~\ref{fig:approach} for a schematic). For a number of low-level textual, speech, and visual features, we analyze how the alignment between brain recordings and language model representations is affected by the elimination of information related to these features. We further contrast our findings with speech-based language models, which would be expected to predict speech-evoked brain activity better, provided they model language processing in the brain well. 
For this purpose, we present a systematic study of the brain alignment across two popular fMRI datasets of naturalistic stories (1-reading, 1-listening) and different natural language processing models (text vs. speech).
We focus on three popular text-based language models (BERT~\citep{devlin2019bert},  GPT2~\citep{radford2019language}, and FLAN-T5~\citep{chung2022scaling}) and two speech-based models (Wav2vec2.0~\citep{baevski2020wav2vec} and Whisper~\citep{radford2022robust})–which have been studied extensively in the NLP-brain alignment literature~\citep{toneva2019interpreting,aw2022training,merlin2022language,oota2022neural,oota2022joint,millet2022toward,vaidya2022self}.
The fMRI recordings are openly
available~\citep{deniz2019representation} and correspond to 6 participants reading and listening to the same naturalistic stories. This dataset is the only one of its kind, in which the participants are observing the same naturalistic stimuli but in two different modalities. It is important that the datasets we analyze have the same stimuli but are presented in two different modalities, because if the stimuli differ between modalities, any observed difference between modalities may be due to the difference in the presented stimuli and not to the difference in sensory modalities. 
We test how eliminating a range of low-level textual (number of letters, number of words, word length, etc.), speech (number of phonemes, Fbank, MFCC, Mel, articulation, phonological features, etc.), and visual features (motion energy) in artificial model representations affects alignment with brain responses.



Using our direct approach, we find that 
both types of language models predict brain responses well both during reading and listening in corresponding early sensory regions in large parts due to low-level stimulus features that are correlated between text and speech (e.g. number of letters and phonemes). In contrast, in later language regions, we find that much of the ability of text-based language models to predict brain responses is retained during both listening and reading even after removing low-level stimulus features, suggesting that text-based language models capture important brain-relevant semantics. However, surprisingly, we find that the impressive predictive performance of speech models in the early auditory cortex is not entirely accounted for by low-level features.
%speech-based language models do not predict additional substantial variance in the late language regions, once low-level stimulus features are removed from the model representations. 
Further, we show that 40-50\% of the explainable variance in the early auditory cortex is left to explain after removing the low-level features. This shows that speech-based models capture additional features that are important for early auditory cortex and understanding these further can help us better understand this part of the brain.
Another surprising result is that, in contrast to the alignment of speech-based models in the early auditory cortex, the alignment in late language regions is almost entirely due to low-level features. The surprise is coming from the fact that the predictive performance of the late language regions is still good and almost on par with text-based models, and also from the fact that several recent works have proposed speech-based models for good models of language in the brain. Our work clearly demonstrates the importance of careful consideration of the reasons behind the alignment that is observed between models and human brain recordings.



%These findings suggest that speech models can be further improved to better reflect brain-like language processing, particularly given that speech is the earliest form of human language.


Our main contributions can be summarized as follows: (i) We employ a direct approach to study the fine-grained aspects of information (i.e., low-level textual, speech, and visual features) in different types of neural language processing models and brains; (ii) We show that both text- and speech-based language models predict brain activity well both during reading and listening. During listening, speech-based models outperform text-based models in the auditory cortex. During reading, both text- and speech-based models have similar brain alignment with the early visual regions. However, the alignment with the late language regions is significantly better for text-based vs. speech-based models both during reading and listening; (iii) Our direct residual approach reveals that low-level stimulus features are the primary contributors underlying the alignment with early visual and auditory regions for both types of models. Specifically, diphones and number of letters are the two features that explain the most variance in brain responses for text-based models, while phonological features explain the most variance for speech-based models. We will make all code available upon publication so that other researchers can reproduce and build on our methodology and findings.



==> preICLR_intro.tex <==
The increasing availability of naturalistic fMRI datasets and the use of large-scale neural models can enable a better understanding of the brain's response to natural stimuli. Despite observed differences in early sensory processing regions between reading and listening~\citep{deniz2019representation}, researchers have shown that text-based language models predict both text-evoked (i.e., reading) and speech-evoked (i.e., listening) brain activity to an impressive degree~\citep{wehbe2014simultaneously,jain2018incorporating,toneva2019interpreting,caucheteux2020language,schrimpf2021neural,antonello2021low,aw2022training,merlin2022language,oota2022joint,oota2022neural}.
Since text-based language models are pretrained on written text~\citep{devlin2019bert,radford2019language,chung2022scaling}, and are particularly well-suited to reading tasks, this raises a question of which stimulus features contribute to these language model representations leading to higher brain predictivity, irrespective of sensory modality (reading vs. listening).


Recently, several researchers have shown that speech-based language models ~\citep{millet2022toward,vaidya2022self,tuckute2022many,oota2023neural,oota2023speech} predict speech-evoked brain activity better within the auditory cortex.
This finding is unsurprising given that speech-based language models~\citep{baevski2020wav2vec,radford2022robust} trained on spoken language, and are likely to perform better in auditory-related tasks. 
Considering that speech represents an earlier form of human language, we would be expected to perform language processing in the brain well similar to text-based language model.
However, given the known differences between reading and listening in the brain, there may also be an effect of differences in language models (text vs. speech) when it comes to processing language during reading and listening.
%have recently been available and employed for different modalities (reading vs. listening), this poses several questions.
%Can the stimulus modality impact the alignment between neural activity and language models in brain encoding studies?
%Which naturalistic fMRI dataset is good for brain encoding? 
%However, the characteristics of the naturalistic fMRI dataset, the quality of the fMRI data, the complexity of the stimuli, the variability in neural responses across participants, and the type of neural model are important
% However, with the multitude of available models and datasets, it can be challenging to pin down what characteristics of such models and datasets contribute to predictivity in the relevant brain regions. What role does stimulus modality (reading vs. listening) play in the study of brain alignment? How does model type (text vs. speech, encoder vs. decoder) affect the resulting alignment? 
Hence, the two-pronged approach of investigating which stimulus features contribute representations during speech and language processing and how different language models capture neural activity in the brain promises to yield deeper insights into both systems.


\begin{figure}[t] 
\centering
%\vspace{-1cm}
\includegraphics[width=0.49\linewidth]{images/Approach_part1.pdf}
\includegraphics[width=0.49\linewidth]{images/Approach_final.pdf}
\caption{Approach to directly test for the effect of low-level stimulus features on the alignment between types
of language model and brain recordings (reading vs. listening).}
\label{fig:approach}
\end{figure}

While the alignment between the two systems have been extensively studied at high-level language regions, it is not yet clear whether and how the
two systems align in their information processing pipeline at low-level sensory regions during reading and listening.
Previous fMRI studies have shown that low-level sensory regions primarily handle unimodal information associated with the initial processing of spoken or written language~\citep{deniz2019representation}. 
Here, we investigated the alignment in low-level sensory regions using two types of neural models.
Text-based models are pretrained on written text~\citep{devlin2019bert,radford2019language,chung2022scaling}, and are particularly well-suited to reading tasks; whereas speech-based models~\citep{baevski2020wav2vec,radford2022robust} are trained on spoken language, and might perform better in auditory tasks. 
This raises two key research questions:
Do low-level sensory processing regions have a role in encoding semantic information? To what extent do neural models predict shared representations within the low-level sensory processing regions during reading and listening?
%Can low-level sensory processing regions maintain modality-invariant representations, regardless of whether the input is textual or auditory in nature?

In contrast, high-level regions are purported to process modality-invariant semantic information~\citep{deniz2019representation}. 
%This has been hypothesized to be because syntax and semantic processing is distributed throughout the language network~\citep{}.
However, it is not clear, whether text and speech-based models process modality invariant semantic information in high-level language regions? 
Considering both low-level sensory and high-level language regions, these findings open up the question of whether model representations contain different types of linguistic/speech/visual information and these types of information are related to different parts of the brain both at low-level sensory and high-level language regions. 

%\textcolor{red}{second question?}

% Previous brain encoding studies on reading and listening fMRI states that sensory regions process unimodal information related to low-level processing of spoken or written language\citep{deniz2019representation}. Further, Text-based models, like those pretrained on written text, may excel in tasks related to reading, while speech models, which are trained on spoken language, may perform better in auditory tasks. This poses several research questions:
% Do the low-level sensory processing areas of the brain encode semantic information?
% What percentage of shared representations predicted by the type of model in both low-level sensory processing regions?
% Is low-level processing sensory regions modality invariant?

Our work aims to examine what these model representations contain different types of information via a direct approach (check Fig.~\ref{fig:approach}). For a number of low-level textual, speech and visual features, we analyze how the alignment between brain recordings and neural model representations is affected by the elimination of information related to each low-level information. 
For this purpose, we present a systematic study of the brain alignment across two popular naturalistic stories fMRI datasets (1-reading, 1-listening) and different natural language processing models (text vs. speech, unidirectional vs. bidirectional).
We focus on three popular language models (BERT~\citep{devlin2019bert},  GPT2~\citep{radford2019language} and FLAN-T5~\citep{chung2022scaling}) and two speech models (Wav2vec2.0~\citep{baevski2020wav2vec} and Whisper~\citep{radford2022robust})–which have both been studied extensively in the NLP-brain alignment literature~\citep{toneva2019interpreting,aw2022training,merlin2022language,oota2022neural,oota2022joint,millet2022toward,vaidya2022self}.
We use a dataset of fMRI recordings that are openly
available~\citep{deniz2019representation} and correspond to 6 participants listening and reading to a same natural story.
We test the effect of a range of low-level linguistic features (number of letters, words, word length, etc,.), speech (number of Phonemes, Fbank, MFCC, Mel, Articulation, Phonological features, etc,.) and visual features (motion energy) and neural model representations is affected by the elimination of information related to each low-level property.

Our initial findings report that both text and speech-based language models predict brain activity best based on the brain regions and choice of stimulus modality.
Specifically, in brain listening, speech models outperform text models in the early auditory cortex.
Surprisingly, in brain reading, both text and speech models have similar brain prediction performance in the early visual areas (V1 and V2).
However, text-based language models outperform speech models in the remaining late language regions irrespective of choice of modality i.e. brain reading or listening. 
Further, we find that the average estimated noise ceiling across participants during listening and reading for the same stimuli is similar, and the normalized predictivity (i.e. the fraction of ceiling the neural model can predict) is similar in the two modalities.

Using the residual approach, we aim to understand the types of information that these language models truly predict in different brain regions.
we make the following observations:
(1) In brain reading and early visual areas, low-level textual features are the biggest contributors in both early visual and visual word form processing area (VWFA) cortices for both text and speech models, and not motion energy. This is because these neural language models do not focus much on visual things since they are not meant to be visual models in the first place.
(2) In brain listening and early auditory areas, indeed both neural representations predict early auditory areas largely because of presence of correlated information related to low-level textual and speech features. However, the additional predictive power of speech-based language models over text models due to the additional information present in these models related to fbank, MFCC, Mel spectrogram and PowSpec features.
% there is an additional info captured in speech models related to fbank, MFCC, and spectrogram that is not available in text models
(3) In the late language regions involved in brain reading and listening, neural text-based models have more information shared beyond low-level stimulus features. In contrast, residual performance of speech models (after removal of low-level speech features such as phonological features) have a higher-drop in performance in late language regions.
 

Our main contributions are as follows:
\begin{itemize}
    \item We propose a direct approach to study the fine-grained aspects (i.e low-level textual, speech and visual features) in types of neural language processing models and brains.
    \item We show that text and speech-based language models predict brain activity best based on the brain regions and choice of stimulus modality. We find that speech models outperform text-based models in the auditory cortex in brain listening. On the other hand, in the context of brain reading, both text and speech models have similar brain prediction performance in the early visual areas.
    \item Detailed residual analysis in brain reading and listening reveal that low-level textual features are biggest contributors in both early visual and auditory sensory-processing areas for both text and speech models. Specifically, DiPhones are the important textual property for text models, while phonological features are important for speech models.

    % In brain listening and early auditory areas, speech models outperform text models, although text models still perform better than chance. This aligns with our expectations since speech models are trained on speech data so expected to capture early auditory information, giving them an advantage over text models.
    % \item  In the context of brain reading and early visual regions, it is surprising that both text and speech models exhibit the same degree of brain predictivity. This suggests the possibility that text models may not fully capture in-terms of brain-relevant information in early visual region. However, we observe that text models show greater brain predictivity than speech models in visual word form processing area.
    % \item In brain listening + reading and late language areas: text models > speech models -> would expect that modality doesnt matter as much, but text models still better for both sensory modalities. -> so text models possibly have better representation of semantics (maybe because trained on more data? Or better performing at language modeling?)

\end{itemize}

We will make all code available upon publication.
